Rewriting History: Repurposing Domain-Specific CGRAs

Coarse-grained reconfigurable arrays (CGRAs) are domain-specific devices promising both the flexibility of FPGAs and the performance of ASICs. However, with restricted domains comes a danger: designing chips that cannot accelerate enough current and future software to justify the hardware cost. We introduce FlexC, the first flexible CGRA compiler, which allows CGRAs to be adapted to operations they do not natively support. FlexC uses dataflow rewriting, replacing unsupported regions of code with equivalent operations that are supported by the CGRA. We use equality saturation, a technique enabling efficient exploration of a large space of rewrite rules, to effectively search through the program-space for supported programs. We applied FlexC to over 2,000 loop kernels, compiling to four different research CGRAs and 300 generated CGRAs and demonstrate a 2.2$\times$ increase in the number of loop kernels accelerated leading to 3$\times$ speedup compared to an Arm A5 CPU on kernels that would otherwise be unsupported by the accelerator.

==> performance_ceiling.tex <==
\subsection{Determining the Performance Ceiling of a CGRA}
%SAM: I'd be inclined to move (some of) this later in the paper. It takes the wind out of the sails of the more technical aspects here. 
Given a space of programs $\mathcal{P}$ and a CGRA $Acc$, \tkcomment{is this a turing-complete space?}
we write the set of programs that $Acc$ supports using
using a particular compiler $C$ as $\text{Supp}_C(Acc) \subseteq \mathcal{P}$.

We say that $Acc$ is domain-specific if $\text{Supp}_C(Acc) \subset \mathcal{P}$ \tkcomment{is this forall compilers? if so how do you know that there exists no compiler that would make $Acc$ general purpose?},
and in practice, for CGRAs we expect $\text{Supp}_C(Acc)$ to be much smaller
than the set of all programs.

\subsubsection{The Performance Ceiling}
As compiling for CGRAs is an NP-complete problem~\cite{TODO},
a complete rewrite exploration (that is, a compiler that always produces a mapping if one exists) isn't practical.  
%SAM: This seems an innocuous statement at first glance, but it really isn't. As the dragon book argues, an optimising compiler for a general-purpose core isn't just NP complete, it's undecidable! So either you're saying that a CGRA compilation is even easier than for a CPU (!), or you're not saying much at all, or you're saying something else.
% The statement is ambiguous: you appear to conflate compilation with optimising compilation. Are you saying that finding any successful compilation, should it exist, is an NP-hard decision problem, maybe? By optimal, do you mean ``produces a solution if it exists'' as opposed to ``produces the most minimal/fastest solution"? I think, on reading later on, you're saying the former -- which I've added in brackets.
% This also brings to the point, that what your input is isn't clear. Is it an entire program, written in E.g. C? Or are your target expressions clearly demarcated, because they're written in some DSL? If not, how do you choose what expression granularity you rewrite at? Is that another design space?
% My fourth objection is along the lines of ``SAT is an NP-hard problem, so no theorem provers exist at all ACTUALLY.'' NP-complete isn't that high of a barrier, and it only implies the need for non-admissible heuristics (which lead away from optimality) in some cases. Are you actually saying that the search space is exponential? Because even that surprises me -- I'd expect it to be infinite in some cases, and the problem to be undecidable (though maybe the shape of the CGRA means the expression size is bounded?)

However, we can quantify
a performance ceiling of an ideal system and consider how close a compiler using heuristics
is to this ceiling.
For some CGRA $Acc$ and space of programs $\mathcal{P}$, we can define an optimal compiler
$C^{\mathit{opt}}$.  The \textit{accuracy} of a heuristic-based compiler,
$C^{\mathit{heur}}$, can be measured relative to this
performance ceiling as the probability that the heuristic returns the same result as the optimal solution (either a true negative or true positive, versus a false negative): \tkcomment{what if it returns a different result with the same performance?}
%SAM: I think that's the most intuitive way of explaining it -- a normal accuracy would include false positives, but they won't exist here, hence why this formula is relevant.

\begin{multline*}
	\mathit{ceil}(\mathit{heur}, Acc) = 
	P(x \in \text{Supp}_{C^{opt}}(Acc) \implies \\ x \in \text{Supp}_{C^{heur}}(Acc) | x \in \mathcal{P})
\end{multline*}
%This is a measure of accuracy, and it's not clear to me that it's the correct measurement to use. Most programs in the world won't match a CGRA -- so does that mean a null heuristic gets 99% benefit because most programs don't match anyway?
%I wonder if the better metric might be a recall metric:
%\begin{align*}
%	\mathit{ceil}(\mathit{heur}, Acc) = 
%	P(x \in \text{Supp}_{C^{heur}}(Acc) |x \in \text{Supp}_{C^{opt}}(Acc) \wedge x \in \mathcal{P})
%\end{align*}
%Can you justify your choice of accuracy instead?
% It's also not clear how a) you would compute this in a meaningful way, b) it isn't just a generic formula you would use for any inadmissible heuristic with no false positives? So it sort-of reads like you're just musing about heuristics in the general, without saying anything.



Figure~\ref{PerformanceCeilingDiagramHomogeneous} shows how the supported
set sizes can be compared against each other.  Each set of programs
corresponds to the set supported by a compiler.

\begin{figure}
	\caption{Different compilation strategies can support different
		numbers of programs within a fixed performance bound: both
		due to optimality of mapping and finding the mapping
	to start with.  }
	\label{PerformanceCeiliingDiagramHomogeneous}
\end{figure}

\subsubsection{The Performance Ceiling in Heterogeneous CGRAs}
We explore the application of rewrite exploration to CGRAs.
In this case, the definition of the ceiling of CGRA support
can be given by considering the set of operations
that a given program can be reduced to.
\tkcomment{why do we start talking about heterogenity and rewriting at the same time? rewriting could also be beneficial for performance on homogeneous hardware}

We define this with respect to an optimal compiler/rule rewriter.
So, for some given ruleset $R$, we can define:

\begin{multline*}
	\mathit{ceil}_R(\mathit{rewriter}, \mathit{heur}, A) = \\
	P(\mathit{OptimalRewriter}_R(x) \in \text{Supp}_{C^{\mathit{opt}}}(A) \implies \\ \mathit{rewriter}_R(x) \in \text{Supp}_{C^{\mathit{heur}}}(A) | x \in \mathcal{P})
\end{multline*}

Where we define $\mathit{OptimalRewriter}_R(x)$ to rewrite $x$ such that
if an equivalent expression in $\text{Supp}_{C^{\mathit{opt}}}(A)$ exists,
it is found by the rewriter. \tkcomment{I'm surprised that rewriting is not part of the compiler: is the compiler only performing data-flow scheduling?}

Figure~\ref{PerformanceCeilingDiagram} shows how using a rewriter
can increase the fraction of programs supported.  In the diagram,
two different sets of rewrite rules are applied to a CGRA
under a particular compiler.  Practical rewriting strategies
can approach the performance ceiling, but due to the exhaustive search
required to achieve the performance ceiling, are often unable to.

\subsection{Practical Estimation of the Performance Ceiling in Heterogeneous CGRA}
TODO

\begin{figure}
	\includegraphics[width=0.45\textwidth]{./Diagrams/ProgramSpaceDiagram-eps-converted-to.pdf}
	\caption{
		More programs can be supported on a particular CGRA using rewrite
		rules to convert operations using the same compilation
		strategy.
		Each set is a different set of rewrite rules, using
		\name{} to generate valid programs. Because the floating-point rules sacrifice precision of the result, both the optimal rewriter and the egraph rewriter potentially cover a larger set than even the optimal rewriter using the GCC rules alone.
	}
%SAM: these are the same picture! It's not clear why you've made a distinction, what the size difference means, or why you'd ever use one set of rules over the other. Perhaps it's to do with the FP rewrites sacrificing correctness? That's what I wrote in the final sentence at least.
	\label{PerformanceCeilingDiagram}
\end{figure}


